Cybersecurity AI (CAI) Dataset

We present CAI Dataset, a fourteen-month corpus of cybersecurity LLM trajectories collected through the open-source CAI agent framework, built in response to PentestGPT's finding that expert operator trajectories, not base-model capability, are the bottleneck for cybersecurity LLM performance. CAI Dataset aggregates 230,935 session logs and 26,027,742 user prompts from 16,768 source IPs across 123 countries, exercising 4,187 unique LLM identifiers against 23,147 target domains over 18.07 TB of durable storage. The mix is hands-on (36.4% offensive, 20.1% attacker-intent, 27.5% business / integration, 4.4% defensive), making CAI Dataset, to the best of our knowledge, the largest described corpus of LLM-driven hacker trajectories. It is released to partner organisations and selected customers as an audience-size series (CAI Dataset10, CAI Dataset1k, CAI Dataset200k). Read longitudinally, the corpus is a record of cybersecurity itself turning automated: operators routinely paste live credentials, production hostnames and bearer tokens into prompts knowing their inputs are logged, a trade-off they accept to stay competitive. Aggregated across the industry, this concentrates a substantial fraction of the world's offensive and defensive operator context inside a handful of frontier-model API providers, a single failure surface whose breach or politically motivated repurposing could cascade into nation- and enterprise-scale disruption. The only configuration that preserves both the productivity advantage and operator-side confidentiality is an on-premise, privately-hosted cybersecurity-specialised LLM served inside the operator's trust boundary, which CAI Dataset is shaped to make practical.

==> tex/world_land_110m.tex <==
% Generated from Natural Earth 1:110m land polygons.
% Source: https://www.naturalearthdata.com/downloads/110m-physical-vectors/110m-land/
% Simplified to 0.55 degrees for compact TikZ/pgfplots rendering.
\addplot[worldland, forget plot]
    coordinates {
        (106.97,76.97) (114.13,75.85) (109.40,74.18) (123.20,72.97) (123.26,73.74) (126.98,73.57) (131.29,70.79) (132.25,71.84)
        (139.87,71.49) (139.15,72.42) (140.47,72.85) (149.50,72.20) (152.97,70.84) (159.00,70.87) (160.94,69.44) (167.84,69.58)
        (169.58,68.69) (170.82,69.01) (170.01,69.65) (170.45,70.10) (175.72,69.88) (180.00,68.96) (180.00,64.98) (177.41,64.61)
        (179.23,62.30) (173.68,61.65) (170.33,59.88) (168.90,60.57) (163.54,59.87) (162.02,58.24) (163.19,57.62) (162.12,54.86)
        (160.37,54.34) (160.02,53.20) (158.53,52.96) (156.79,51.01) (155.43,55.38) (155.91,56.77) (163.67,61.14) (164.47,62.55)
        (160.12,60.54) (159.30,61.77) (156.72,61.43) (154.22,59.76) (155.04,59.15) (151.27,58.78) (151.34,59.50) (149.78,59.66)
        (142.20,59.04) (135.13,54.73) (138.16,53.76) (139.90,54.19) (141.38,52.24) (140.06,48.45) (138.22,46.31) (134.87,43.40)
        (132.28,43.28) (127.53,39.76) (129.46,36.78) (129.09,35.08) (126.49,34.39) (126.12,36.73) (126.86,36.89) (124.71,38.11)
        (125.32,39.55) (121.05,38.90) (122.17,40.42) (121.64,40.95) (118.04,39.20) (117.53,38.74) (118.91,37.45) (122.36,37.45)
        (119.15,34.91) (121.91,31.69) (121.26,30.68) (122.09,29.83) (121.68,28.23) (118.66,24.55) (115.89,22.78) (110.79,21.40)
        (110.44,20.34) (108.52,21.72) (105.88,19.75) (109.34,13.43) (109.20,11.67) (105.16,8.60) (105.08,9.92) (100.10,13.41)
        (99.22,9.24) (102.96,5.52) (104.23,1.29) (101.39,2.76) (100.09,6.46) (98.50,8.38) (98.34,7.79) (98.76,11.44)
        (97.16,16.93) (95.37,15.71) (94.19,16.04) (94.32,18.21) (91.42,22.77) (90.50,22.81) (90.27,21.84) (86.98,21.50)
        (86.50,20.15) (80.32,15.90) (79.86,10.36) (77.54,7.97) (73.53,15.99) (72.63,21.36) (70.47,20.88) (66.37,25.43)
        (57.40,25.74) (56.49,27.14) (54.72,26.48) (51.52,27.87) (50.12,30.15) (47.97,29.98) (50.81,24.75) (51.01,26.01)
        (51.59,25.80) (51.79,24.02) (54.01,24.12) (56.36,26.40) (56.85,24.24) (59.81,22.31) (57.83,20.24) (57.69,18.94)
        (55.27,17.23) (48.68,14.00) (43.48,12.64) (42.65,16.77) (39.14,21.29) (38.49,23.69) (34.63,28.06) (34.92,29.50)
        (33.92,27.65) (32.42,29.85) (35.53,23.10) (36.87,22.00) (37.48,18.61) (43.32,12.39) (42.72,11.74) (44.61,10.44)
        (51.11,12.02) (51.05,10.64) (47.74,4.22) (40.26,-2.57) (39.20,-4.68) (38.80,-6.48) (40.48,-10.77) (40.78,-14.69)
        (39.45,-16.72) (34.79,-19.78) (35.61,-23.71) (32.57,-25.73) (32.20,-28.75) (28.22,-32.77) (25.78,-33.94) (19.62,-34.82)
        (18.38,-34.14) (18.22,-31.66) (15.21,-27.09) (14.26,-22.11) (11.79,-18.07) (11.78,-15.79) (13.69,-10.73) (11.92,-5.04)
        (8.80,-1.11) (9.40,3.73) (8.50,4.77) (5.90,4.26) (4.33,6.27) (-1.96,4.71) (-9.00,4.83) (-12.43,7.26)
        (-16.61,12.17) (-17.62,14.73) (-16.15,18.11) (-16.97,21.89) (-14.44,26.25) (-9.56,29.93) (-9.30,32.56) (-5.93,35.76)
        (-2.17,35.17) (1.47,36.61) (9.51,37.35) (11.10,36.90) (10.34,33.79) (19.09,30.27) (20.13,32.24) (21.54,32.84)
        (28.91,30.87) (30.98,31.56) (33.77,30.97) (36.00,34.64) (36.16,36.65) (27.64,36.66) (26.17,39.46) (29.24,41.22)
        (33.51,42.02) (38.35,40.95) (41.70,41.96) (36.68,45.24) (39.12,47.26) (34.96,46.27) (36.33,45.11) (33.88,44.36)
        (32.45,45.33) (33.30,46.08) (30.75,46.58) (27.67,42.58) (28.81,41.05) (26.36,40.15) (24.93,40.95) (23.71,40.69)
        (23.90,39.96) (22.63,40.26) (24.04,37.66) (23.12,37.92) (23.15,36.42) (22.49,36.41) (19.41,40.25) (19.54,41.72)
        (13.14,45.74) (12.33,45.38) (12.59,44.09) (18.48,40.17) (16.87,40.44) (17.05,38.90) (16.10,37.99) (15.41,40.05)
        (8.89,44.37) (6.53,43.13) (3.10,43.08) (3.04,41.89) (0.81,41.01) (0.11,38.74) (-2.15,36.67) (-5.38,35.95)
        (-6.52,36.94) (-8.90,36.87) (-9.39,43.03) (-1.38,44.02) (-1.19,46.01) (-4.59,48.68) (-1.62,48.64) (-1.93,49.78)
        (1.34,50.13) (4.71,53.09) (8.12,53.53) (8.80,54.02) (8.12,55.52) (8.54,57.11) (10.58,57.73) (10.91,56.46)
        (9.65,55.47) (10.94,54.01) (19.66,54.43) (21.27,55.19) (21.58,57.41) (24.12,57.03) (24.43,58.38) (23.34,59.19)
        (29.12,60.03) (22.87,59.85) (21.32,60.72) (21.54,63.19) (25.40,65.11) (23.90,66.01) (22.18,65.72) (21.37,64.41)
        (17.85,62.75) (17.12,61.34) (18.79,60.08) (16.83,58.72) (15.88,56.10) (12.94,55.36) (10.36,59.47) (8.38,58.31)
        (5.67,58.59) (4.99,61.97) (10.53,64.49) (14.76,67.81) (24.55,71.03) (28.17,71.19) (31.29,70.45) (30.01,70.19)
        (31.10,69.56) (36.51,69.06) (41.06,67.46) (41.13,66.79) (38.38,66.00) (33.18,66.63) (34.81,65.90) (34.94,64.41)
        (37.01,63.85) (36.52,64.78) (37.18,65.14) (39.59,64.52) (40.44,64.76) (39.76,65.50) (42.09,66.48) (43.95,66.07)
        (44.53,66.76) (43.45,68.57) (46.25,68.25) (46.82,67.69) (45.56,67.01) (46.35,66.67) (53.72,68.86) (54.47,68.81)
        (53.49,68.20) (58.80,68.88) (59.94,68.28) (61.08,68.94) (60.03,69.52) (60.55,69.85) (68.51,68.09) (69.18,68.62)
        (66.93,69.45) (66.69,71.03) (69.20,72.84) (72.59,72.78) (71.85,71.41) (72.79,70.39) (72.56,69.02) (73.67,68.41)
        (71.28,66.32) (72.42,66.17) (75.05,67.76) (74.94,68.99) (73.60,69.63) (74.40,70.63) (73.10,71.45) (74.89,72.12)
        (74.66,72.83) (75.68,72.30) (75.29,71.34) (76.36,71.15) (75.90,71.87) (77.58,72.27) (81.50,71.75) (80.51,73.65)
        (86.82,73.94) (86.01,74.46) (87.17,75.12) (106.07,77.37) (104.71,77.13) (106.97,76.97)
    }; % land 1
\addplot[worldland, forget plot]
    coordinates {
        (-90.55,69.50) (-90.55,68.48) (-89.22,69.26) (-87.35,67.20) (-85.58,68.78) (-85.52,69.88) (-82.62,69.66) (-81.28,69.16)
        (-81.96,68.13) (-81.26,67.60) (-83.34,66.41) (-85.77,66.56) (-87.32,64.78) (-93.16,62.02) (-94.68,58.95) (-93.22,58.78)
        (-92.30,57.09) (-82.27,55.15) (-82.12,53.28) (-79.91,51.21) (-78.60,52.56) (-79.83,54.67) (-76.54,56.53) (-78.52,58.80)
        (-77.34,59.85) (-78.11,62.32) (-73.84,62.44) (-69.59,61.06) (-69.29,58.96) (-67.65,58.21) (-64.58,60.34) (-61.40,56.97)
        (-61.80,56.34) (-57.33,54.63) (-55.76,53.27) (-55.68,52.15) (-60.03,50.24) (-66.40,50.23) (-71.10,46.82) (-65.06,49.23)
        (-64.17,48.74) (-65.12,48.07) (-64.47,46.24) (-61.52,45.88) (-60.52,47.01) (-59.80,45.92) (-65.36,43.55) (-66.16,44.47)
        (-64.43,45.29) (-67.14,45.14) (-70.69,43.03) (-69.97,41.64) (-73.71,40.93) (-71.95,40.93) (-73.95,40.75) (-74.91,38.94)
        (-75.53,39.50) (-75.06,38.40) (-75.94,37.22) (-76.35,39.15) (-76.33,38.08) (-76.96,38.23) (-75.73,35.55) (-81.34,31.44)
        (-80.06,26.88) (-80.38,25.21) (-81.71,25.87) (-84.10,30.09) (-89.18,30.32) (-89.22,29.29) (-90.15,29.12) (-93.85,29.71)
        (-96.59,28.31) (-97.37,27.38) (-97.87,22.44) (-96.29,19.32) (-94.43,18.14) (-92.04,18.70) (-90.77,19.28) (-90.28,21.00)
        (-87.05,21.54) (-88.93,15.89) (-83.41,15.27) (-83.81,11.10) (-81.44,8.79) (-79.57,9.61) (-76.84,8.64) (-74.91,11.08)
        (-71.75,12.44) (-71.14,12.11) (-71.95,11.42) (-71.70,9.07) (-71.40,10.97) (-69.94,12.16) (-68.19,10.55) (-64.89,10.08)
        (-61.88,10.72) (-62.39,9.95) (-57.15,5.97) (-53.96,5.76) (-51.32,4.20) (-49.97,1.74) (-50.39,-0.08) (-48.62,-0.24)
        (-48.58,-1.24) (-47.82,-0.58) (-44.91,-1.55) (-44.58,-2.69) (-39.98,-2.87) (-35.60,-5.15) (-34.73,-7.34) (-35.13,-9.00)
        (-38.67,-13.06) (-39.27,-17.87) (-40.94,-21.94) (-47.65,-24.89) (-48.89,-28.67) (-53.81,-34.40) (-56.22,-34.86) (-58.43,-33.91)
        (-56.79,-36.90) (-59.23,-38.72) (-62.34,-38.83) (-62.75,-41.03) (-65.12,-41.06) (-64.98,-42.06) (-63.46,-42.56) (-65.18,-43.50)
        (-65.57,-45.04) (-67.29,-45.55) (-67.58,-46.30) (-65.64,-47.24) (-65.99,-48.13) (-69.14,-50.73) (-68.15,-52.35) (-70.85,-52.90)
        (-71.01,-53.83) (-74.95,-52.26) (-75.61,-48.67) (-74.13,-46.94) (-75.64,-46.65) (-74.35,-44.10) (-73.24,-44.45) (-72.72,-42.38)
        (-74.33,-43.22) (-73.22,-39.26) (-73.59,-37.16) (-71.44,-32.42) (-70.16,-19.76) (-71.46,-17.36) (-76.01,-14.65) (-79.76,-7.19)
        (-81.25,-6.14) (-81.41,-4.74) (-79.77,-2.66) (-80.97,-2.25) (-80.93,-1.06) (-77.13,3.85) (-78.18,8.32) (-79.56,8.93)
        (-80.89,7.22) (-85.66,9.93) (-87.49,13.30) (-91.23,13.93) (-94.69,16.20) (-96.56,15.65) (-103.50,18.29) (-105.49,19.95)
        (-106.03,22.77) (-112.23,28.95) (-113.15,31.17) (-114.78,31.80) (-114.67,30.16) (-109.43,23.19) (-110.03,22.82) (-112.18,24.74)
        (-112.30,26.01) (-115.06,27.72) (-114.16,28.57) (-117.30,33.05) (-120.62,34.61) (-124.40,40.31) (-123.90,45.52) (-124.69,48.18)
        (-123.12,48.04) (-122.59,47.10) (-122.84,49.00) (-127.44,50.83) (-127.85,52.33) (-129.13,52.76) (-134.08,58.12) (-147.11,60.88)
        (-151.72,59.16) (-150.62,61.28) (-154.02,59.35) (-153.29,58.86) (-154.23,58.15) (-158.43,55.99) (-164.79,54.40) (-157.72,57.57)
        (-157.04,58.92) (-161.97,58.67) (-161.87,59.63) (-163.82,59.80) (-166.12,61.50) (-164.56,63.15) (-160.77,63.77) (-161.52,64.40)
        (-160.78,64.79) (-164.96,64.45) (-168.11,65.67) (-164.47,66.58) (-161.68,66.12) (-166.76,68.36) (-156.58,71.36) (-136.50,68.90)
        (-128.14,70.48) (-125.76,69.48) (-124.42,70.16) (-124.29,69.40) (-121.47,69.80) (-113.90,68.40) (-115.30,67.90) (-108.88,67.38)
        (-107.79,67.89) (-108.81,68.31) (-108.17,68.65) (-106.15,68.80) (-101.45,67.65) (-98.44,67.78) (-97.67,68.58) (-96.12,68.24)
        (-96.13,67.29) (-94.23,69.07) (-96.47,70.09) (-96.39,71.19) (-95.21,71.92) (-91.52,70.19) (-92.41,69.70) (-90.55,69.50)
    }; % land 2
\addplot[worldland, forget plot]
    coordinates {
        (143.56,-13.76) (145.37,-14.98) (146.39,-18.96) (148.85,-20.39) (153.14,-26.07) (152.89,-31.64) (150.00,-37.43) (146.32,-39.04)
        (145.03,-37.90) (143.61,-38.81) (140.64,-38.02) (139.57,-36.14) (138.12,-35.61) (138.21,-34.38) (136.83,-35.26) (137.81,-32.90)
        (135.99,-34.89) (134.27,-32.62) (131.33,-31.50) (126.15,-32.22) (123.66,-33.89) (119.89,-33.98) (118.02,-35.06) (115.03,-34.20)
        (115.69,-31.61) (113.34,-26.12) (114.23,-26.30) (113.39,-24.38) (114.15,-21.76) (114.23,-22.52) (116.71,-20.70) (120.86,-19.68)
        (123.01,-16.41) (123.86,-17.07) (123.50,-16.60) (125.69,-14.23) (127.07,-13.82) (129.62,-14.97) (130.62,-12.54) (132.58,-12.11)
        (131.82,-11.27) (136.49,-11.86) (136.95,-12.35) (135.50,-15.00) (140.22,-17.71) (141.27,-16.39) (142.52,-10.67) (143.60,-13.40)
        (143.56,-13.76)
    }; % land 3
\addplot[worldland, forget plot]
    coordinates {
        (-27.10,83.52) (-20.85,82.73) (-31.90,82.20) (-22.07,81.73) (-23.17,81.15) (-15.77,81.91) (-12.21,81.29) (-20.05,80.18)
        (-17.73,80.13) (-19.70,78.75) (-19.67,77.64) (-18.47,76.99) (-21.68,76.63) (-19.83,76.10) (-19.60,75.25) (-20.67,75.16)
        (-19.37,74.30) (-23.57,73.31) (-22.30,72.18) (-24.79,72.33) (-21.75,70.66) (-25.54,71.43) (-25.20,70.75) (-26.36,70.23)
        (-22.35,70.13) (-39.81,65.46) (-42.82,62.68) (-42.42,61.90) (-43.38,60.10) (-48.26,60.86) (-51.63,63.63) (-53.97,67.19)
        (-50.87,69.93) (-54.68,69.61) (-54.36,70.82) (-51.39,70.57) (-55.83,71.65) (-54.72,72.59) (-58.59,75.52) (-68.50,76.06)
        (-71.40,77.01) (-66.76,77.38) (-73.30,78.04) (-65.71,79.39) (-68.02,80.12) (-62.23,81.32) (-62.65,81.77) (-50.39,82.44)
        (-44.52,81.66) (-46.76,82.63) (-35.09,83.65) (-27.10,83.52)
    }; % land 4
\addplot[worldland, forget plot]
    coordinates {
        (-86.56,73.16) (-85.77,72.53) (-82.32,73.75) (-80.60,72.72) (-80.75,72.06) (-77.82,72.75) (-74.10,71.33) (-72.24,71.56)
        (-66.97,69.19) (-68.81,68.72) (-61.85,66.86) (-63.92,65.00) (-68.02,66.26) (-64.67,63.39) (-65.01,62.67) (-68.78,63.75)
        (-66.17,61.93) (-74.83,64.68) (-77.71,64.23) (-78.56,64.57) (-77.90,65.31) (-73.96,65.45) (-72.93,67.73) (-78.96,70.17)
        (-84.94,69.97) (-89.89,71.22) (-89.44,73.13) (-85.83,73.80) (-86.56,73.16)
    }; % land 5
\addplot[worldland, forget plot]
    coordinates {
        (-68.50,83.11) (-61.85,82.63) (-67.66,81.50) (-65.48,81.51) (-71.18,79.80) (-76.91,79.32) (-75.39,78.53) (-79.76,77.21)
        (-77.89,76.78) (-80.56,76.18) (-89.49,76.47) (-87.77,77.18) (-88.26,77.90) (-84.98,77.54) (-87.96,78.37) (-85.09,79.35)
        (-86.93,80.25) (-81.85,80.46) (-87.60,80.52) (-91.59,81.89) (-70.67,83.17) (-68.50,83.11)
    }; % land 6
\addplot[worldland, forget plot]
    coordinates {
        (134.14,-1.15) (134.42,-2.77) (135.46,-3.37) (138.33,-1.70) (144.58,-3.86) (147.65,-6.08) (147.19,-7.39) (150.69,-10.58)
        (147.91,-10.13) (144.74,-7.63) (142.63,-9.33) (139.13,-8.10) (137.61,-8.41) (138.67,-7.32) (137.93,-5.39) (133.66,-3.54)
        (132.98,-4.11) (131.99,-2.82) (133.70,-2.21) (130.52,-0.94) (133.99,-0.78) (134.14,-1.15)
    }; % land 7
\addplot[worldland, forget plot]
    coordinates {
        (117.88,1.83) (119.00,0.90) (117.81,0.78) (116.15,-4.01) (110.22,-2.93) (109.09,-0.46) (109.66,2.01) (111.17,1.85)
        (111.37,2.70) (113.00,3.10) (116.73,6.92) (119.18,5.41) (117.31,3.23) (118.05,2.29) (117.88,1.83)
    }; % land 8
\addplot[worldland, forget plot]
    coordinates {
        (-114.17,73.12) (-114.67,72.65) (-109.92,72.96) (-108.19,71.65) (-107.69,72.07) (-108.40,73.09) (-106.52,73.08) (-104.46,70.99)
        (-101.09,69.58) (-102.73,69.50) (-102.43,68.75) (-113.31,68.54) (-117.34,69.96) (-112.42,70.37) (-117.90,70.54) (-118.43,70.91)
        (-116.11,71.31) (-119.40,71.56) (-115.19,73.31) (-114.17,73.12)
    }; % land 9
\addplot[worldland, forget plot]
    coordinates {
        (50.06,-13.56) (50.38,-15.71) (49.67,-15.71) (47.10,-24.94) (45.41,-25.60) (44.04,-24.99) (43.25,-22.06) (44.37,-20.07)
        (44.45,-16.22) (47.71,-14.59) (49.19,-12.04) (49.81,-12.90) (50.06,-13.56)
    }; % land 10
\addplot[worldland, forget plot]
    coordinates {
        (49.11,41.28) (50.39,40.26) (48.86,38.82) (49.20,37.58) (53.83,36.97) (53.88,38.95) (52.69,40.03) (52.92,40.88)
        (54.74,40.95) (53.72,42.12) (52.81,41.14) (52.50,42.79) (50.31,44.61) (53.04,45.26) (53.04,46.85) (49.10,46.40)
        (46.68,44.61) (48.58,41.81) (49.11,41.28)
    }; % land 11
\addplot[worldland, forget plot]
    coordinates {
        (105.82,-5.85) (102.58,-4.22) (95.29,5.48) (97.48,5.25) (100.64,2.10) (102.50,1.40) (103.84,0.10) (103.44,-0.71)
        (106.11,-3.06) (105.86,-4.31) (105.82,-5.85)
    }; % land 12
\addplot[worldland, forget plot]
    coordinates {
        (-3.01,58.64) (-4.07,57.55) (-1.96,57.68) (-3.12,55.97) (1.68,52.74) (1.45,51.29) (-5.25,49.96) (-5.78,50.16)
        (-3.41,51.43) (-5.27,51.99) (-4.22,52.30) (-4.58,53.50) (-2.95,53.98) (-4.84,54.79) (-5.05,55.78) (-5.59,55.31)
        (-6.15,56.79) (-5.01,58.63) (-4.21,58.55) (-3.01,58.64)
    }; % land 13
\addplot[worldland, forget plot]
    coordinates {
        (140.98,37.14) (140.25,35.14) (137.22,34.61) (135.79,33.46) (135.08,34.60) (130.99,33.89) (132.00,33.15) (131.33,31.45)
        (130.20,31.42) (130.45,32.32) (129.41,33.30) (132.62,35.43) (135.68,35.53) (136.72,37.30) (137.39,36.83) (139.43,38.22)
        (139.88,40.56) (141.37,41.38) (141.88,39.18) (140.96,38.17) (140.98,37.14)
    }; % land 14
\addplot[worldland, forget plot]
    coordinates {
        (57.54,70.72) (53.68,70.76) (51.46,72.01) (55.63,75.08) (61.17,76.25) (68.85,76.54) (58.48,74.31) (55.42,72.37)
        (55.62,71.54) (57.54,70.72)
    }; % land 15
\addplot[worldland, forget plot]
    coordinates {
        (-175.01,66.58) (-171.86,66.91) (-169.90,65.98) (-172.53,65.44) (-172.96,64.25) (-178.36,65.39) (-178.69,66.11) (-179.88,65.87)
        (-180.00,64.98) (-180.00,68.96) (-174.93,67.21) (-175.01,66.58)
    }; % land 16
\addplot[worldland, forget plot]
    coordinates {
        (-14.51,66.46) (-14.74,65.81) (-13.61,65.13) (-18.66,63.50) (-22.76,63.96) (-21.78,64.40) (-23.96,64.89) (-22.23,65.38)
        (-24.33,65.61) (-23.65,66.26) (-20.58,65.73) (-16.17,66.53) (-14.51,66.46)
    }; % land 17
\addplot[worldland, forget plot]
    coordinates {
        (18.25,79.70) (21.54,78.96) (15.91,76.77) (10.44,79.65) (16.99,80.05) (18.25,79.70)
    }; % land 18
\addplot[worldland, forget plot]
    coordinates {
        (-120.46,71.40) (-123.09,70.90) (-125.93,71.87) (-123.94,73.68) (-124.92,74.29) (-115.51,73.48) (-120.46,71.82) (-120.46,71.40)
    }; % land 19
\addplot[worldland, forget plot]
    coordinates {
        (-87.02,79.66) (-85.81,79.34) (-90.80,78.22) (-96.71,80.16) (-92.41,81.26) (-87.81,80.32) (-87.02,79.66)
    }; % land 20
\addplot[worldland, forget plot]
    coordinates {
        (173.02,-40.92) (174.25,-41.35) (173.08,-43.85) (171.45,-44.24) (169.33,-46.64) (166.68,-46.22) (167.05,-45.11) (170.52,-43.03)
        (172.80,-40.49) (173.02,-40.92)
    }; % land 21
\addplot[worldland, forget plot]
    coordinates {
        (125.24,1.42) (123.69,0.24) (120.18,0.24) (120.94,-1.41) (123.34,-0.62) (121.51,-1.90) (123.16,-5.34) (122.24,-5.28)
        (122.72,-4.46) (121.49,-4.57) (120.97,-2.63) (120.31,-2.93) (120.43,-5.53) (119.37,-5.38) (119.50,-3.49) (118.77,-2.80)
        (120.04,0.57) (125.07,1.64) (125.24,1.42)
    }; % land 22
\addplot[worldland, forget plot]
    coordinates {
        (-56.13,50.69) (-56.80,49.81) (-53.48,49.25) (-53.79,48.52) (-53.09,48.69) (-52.65,47.54) (-53.07,46.66) (-54.18,46.81)
        (-54.24,47.75) (-55.40,46.88) (-56.25,47.63) (-59.27,47.60) (-57.36,50.72) (-55.60,51.32) (-56.13,50.69)
    }; % land 23
\addplot[worldland, forget plot]
    coordinates {
        (-94.68,77.10) (-89.19,75.61) (-81.13,75.71) (-79.83,74.92) (-92.42,74.84) (-92.89,75.88) (-97.12,76.75) (-96.75,77.16)
        (-94.68,77.10)
    }; % land 24
\addplot[worldland, forget plot]
    coordinates {
        (99.94,78.88) (94.97,79.04) (91.18,80.34) (95.94,81.25) (100.19,79.78) (99.94,78.88)
    }; % land 25
\addplot[worldland, forget plot]
    coordinates {
        (-108.21,76.20) (-105.70,75.48) (-112.22,74.42) (-113.87,74.72) (-111.79,75.16) (-117.71,75.22) (-115.40,76.48) (-109.07,75.47)
        (-110.50,76.43) (-108.55,76.68) (-108.21,76.20)
    }; % land 26
\addplot[worldland, forget plot]
    coordinates {
        (174.61,-36.16) (176.76,-37.88) (178.52,-37.70) (175.24,-41.69) (174.90,-39.91) (173.82,-39.51) (174.70,-37.38) (172.64,-34.53)
        (174.33,-35.27) (174.61,-36.16)
    }; % land 27
\addplot[worldland, forget plot]
    coordinates {
        (121.32,18.50) (122.25,18.48) (122.52,17.09) (121.73,14.33) (123.95,13.78) (124.08,12.54) (120.63,13.86) (119.88,16.36)
        (120.72,18.51) (121.32,18.50)
    }; % land 28
\addplot[worldland, forget plot]
    coordinates {
        (143.91,44.17) (145.32,44.38) (145.54,43.26) (143.18,42.00) (141.61,42.68) (141.07,41.58) (139.96,41.57) (139.82,42.56)
        (141.38,43.39) (141.97,45.55) (143.14,44.51) (143.91,44.17)
    }; % land 29
\addplot[worldland, forget plot]
    coordinates {
        (143.65,50.75) (144.65,48.98) (143.17,49.31) (142.56,47.86) (143.51,46.14) (142.75,46.74) (142.09,45.97) (141.59,51.94)
        (142.21,54.23) (143.24,51.76) (143.65,50.75)
    }; % land 30
\addplot[worldland, forget plot]
    coordinates {
        (-67.75,-53.85) (-65.05,-54.70) (-69.23,-55.50) (-74.66,-52.84) (-71.11,-54.07) (-69.35,-52.52) (-68.25,-53.10) (-67.75,-53.85)
    }; % land 31
\addplot[worldland, forget plot]
    coordinates {
        (-100.36,73.84) (-97.38,73.76) (-98.05,72.99) (-96.54,72.56) (-96.72,71.66) (-99.32,71.36) (-102.50,72.51) (-100.44,72.71)
        (-101.54,73.36) (-100.36,73.84)
    }; % land 32
\addplot[worldland, forget plot]
    coordinates {
        (145.09,75.56) (144.30,74.82) (138.96,74.61) (136.97,75.26) (137.51,75.95) (141.47,76.09) (145.09,75.56)
    }; % land 33
\addplot[worldland, forget plot]
    coordinates {
        (-6.79,52.26) (-9.98,51.82) (-9.17,52.86) (-9.69,53.88) (-6.73,55.17) (-5.66,54.55) (-6.03,53.15) (-6.79,52.26)
    }; % land 34
\addplot[worldland, forget plot]
    coordinates {
        (-85.16,65.66) (-80.10,63.73) (-87.22,63.54) (-85.88,65.74) (-85.16,65.66)
    }; % land 35
\addplot[worldland, forget plot]
    coordinates {
        (-79.68,22.77) (-74.18,20.28) (-77.76,19.86) (-77.09,20.41) (-78.72,21.60) (-81.80,22.64) (-84.97,21.90) (-83.27,22.98)
        (-80.62,23.11) (-79.68,22.77)
    }; % land 36
\addplot[worldland, forget plot]
    coordinates {
        (126.38,8.41) (126.54,7.19) (126.20,6.27) (125.83,7.29) (125.36,6.79) (125.40,5.58) (124.22,6.16) (123.61,7.83)
        (121.92,7.19) (123.49,8.69) (125.47,8.99) (125.41,9.76) (126.31,8.78) (126.38,8.41)
    }; % land 37
\addplot[worldland, forget plot]
    coordinates {
        (108.62,-6.78) (110.76,-6.47) (115.71,-8.37) (105.37,-6.85) (106.05,-5.90) (108.49,-6.42) (108.62,-6.78)
    }; % land 38
\addplot[worldland, forget plot]
    coordinates {
        (145.40,-40.79) (148.29,-40.88) (147.91,-43.21) (146.05,-43.55) (144.74,-40.70) (145.40,-40.79)
    }; % land 39
\addplot[worldland, forget plot]
    coordinates {
        (25.45,80.41) (27.41,80.06) (23.02,79.40) (17.37,80.32) (22.92,80.66) (25.45,80.41)
    }; % land 40
\addplot[worldland, forget plot]
    coordinates {
        (-93.20,72.77) (-95.41,72.06) (-96.02,73.44) (-94.50,74.13) (-90.51,73.86) (-92.00,72.97) (-93.20,72.77)
    }; % land 41
\addplot[worldland, forget plot]
    coordinates {
        (-72.58,19.87) (-68.32,18.61) (-70.67,18.43) (-71.40,17.60) (-73.92,18.03) (-74.37,18.66) (-72.33,18.67) (-73.19,19.92)
        (-72.58,19.87)
    }; % land 42
\addplot[worldland, forget plot]
    coordinates {
        (-98.50,76.72) (-97.74,76.26) (-98.16,75.00) (-102.50,75.56) (-102.57,76.34) (-98.58,76.59) (-98.50,76.72)
    }; % land 43
\addplot[worldland, forget plot]
    coordinates {
        (105.08,78.31) (99.44,77.92) (102.09,79.35) (105.37,78.71) (105.08,78.31)
    }; % land 44
\addplot[worldland, forget plot]
    coordinates {
        (81.22,6.20) (79.87,6.76) (80.15,9.82) (81.79,7.52) (81.64,6.48) (81.22,6.20)
    }; % land 45
\addplot[worldland, forget plot]
    coordinates {
        (-100.06,78.32) (-99.67,77.91) (-105.18,78.38) (-104.21,78.68) (-105.49,79.30) (-100.83,78.80) (-100.06,78.32)
    }; % land 46
\addplot[worldland, forget plot]
    coordinates {
        (-116.20,77.65) (-117.11,76.53) (-122.85,76.12) (-117.57,77.50) (-116.20,77.65)
    }; % land 47
\addplot[worldland, forget plot]
    coordinates {
        (151.98,-5.48) (150.24,-6.32) (148.32,-5.75) (150.81,-5.46) (151.54,-4.17) (152.32,-4.87) (151.98,-5.48)
    }; % land 48
\addplot[worldland, forget plot]
    coordinates {
        (121.18,22.79) (120.75,21.97) (120.11,23.56) (121.50,25.30) (121.78,24.39) (121.18,22.79)
    }; % land 49
\addplot[worldland, forget plot]
    coordinates {
        (15.52,38.23) (15.10,36.62) (12.43,37.61) (14.76,38.14) (15.52,38.23)
    }; % land 50
\addplot[worldland, forget plot]
    coordinates {
        (-123.51,48.51) (-128.44,50.54) (-125.76,50.30) (-123.92,49.06) (-123.51,48.51)
    }; % land 51
\addplot[worldland, forget plot]
    coordinates {
        (51.14,80.55) (47.59,80.01) (44.85,80.59) (51.52,80.70) (51.14,80.55)
    }; % land 52
\addplot[worldland, forget plot]
    coordinates {
        (110.34,18.68) (108.66,18.51) (108.63,19.37) (110.79,20.08) (110.57,19.26) (110.34,18.68)
    }; % land 53
\addplot[worldland, forget plot]
    coordinates {
        (128.69,1.13) (128.10,-0.90) (127.40,1.01) (127.93,2.17) (128.59,1.54) (128.69,1.13)
    }; % land 54
\addplot[worldland, forget plot]
    coordinates {
        (9.21,41.21) (9.67,39.18) (8.81,38.91) (8.16,40.95) (8.71,40.90) (9.21,41.21)
    }; % land 55
\addplot[worldland, forget plot]
    coordinates {
        (-95.65,69.11) (-99.80,69.40) (-98.22,70.14) (-96.26,69.49) (-95.65,69.11)
    }; % land 56
\addplot[worldland, forget plot]
    coordinates {
        (125.50,12.16) (125.78,11.05) (125.01,11.31) (124.80,10.13) (124.27,12.56) (125.23,12.54) (125.50,12.16)
    }; % land 57
\addplot[worldland, forget plot]
    coordinates {
        (124.44,-10.14) (123.46,-10.24) (125.09,-8.66) (127.34,-8.40) (125.09,-9.39) (124.44,-10.14)
    }; % land 58
\addplot[worldland, forget plot]
    coordinates {
        (130.47,-3.09) (130.83,-3.86) (127.90,-3.39) (129.37,-2.80) (130.47,-3.09)
    }; % land 59
\addplot[worldland, forget plot]
    coordinates {
        (-95.83,78.06) (-98.12,78.08) (-98.63,78.87) (-95.56,78.42) (-95.83,78.06)
    }; % land 60
\addplot[worldland, forget plot]
    coordinates {
        (134.64,34.15) (134.20,33.20) (132.36,32.99) (133.90,34.36) (134.64,34.15)
    }; % land 61
\addplot[worldland, forget plot]
    coordinates {
        (123.98,10.28) (123.00,9.02) (122.38,9.71) (124.08,11.23) (123.98,10.28)
    }; % land 62
\addplot[worldland, forget plot]
    coordinates {
        (70.28,-49.71) (68.75,-49.77) (68.94,-48.63) (70.56,-49.26) (70.28,-49.71)
    }; % land 63
\addplot[worldland, forget plot]
    coordinates {
        (-75.87,67.15) (-77.24,67.59) (-75.90,68.29) (-75.22,67.44) (-75.87,67.15)
    }; % land 64
\addplot[worldland, forget plot]
    coordinates {
        (24.72,77.85) (20.73,77.68) (21.42,77.94) (20.81,78.25) (23.28,78.08) (24.72,77.85)
    }; % land 65
\addplot[worldland, forget plot]
    coordinates {
        (118.50,9.32) (117.17,8.37) (119.51,11.37) (119.03,10.00) (118.50,9.32)
    }; % land 66
\addplot[worldland, forget plot]
    coordinates {
        (-104.50,73.42) (-105.38,72.76) (-106.94,73.46) (-105.26,73.64) (-104.50,73.42)
    }; % land 67
\addplot[worldland, forget plot]
    coordinates {
        (-76.34,73.10) (-80.88,73.33) (-78.06,73.65) (-76.34,73.10)
    }; % land 68
\addplot[worldland, forget plot]
    coordinates {
        (12.69,55.61) (12.09,54.80) (11.04,55.36) (12.37,56.11) (12.69,55.61)
    }; % land 69
\addplot[worldland, forget plot]
    coordinates {
        (-153.01,57.12) (-154.01,56.73) (-154.67,57.46) (-152.14,57.59) (-153.01,57.12)
    }; % land 70

